Crosstalk-induced Side Channel Threats in Multi-Tenant NISQ Computers

As quantum computing rapidly advances, its near-term applications are becoming increasingly evident. However, the high cost and under-utilization of quantum resources are prompting a shift from single-user to multi-user access models. In a multi-tenant environment, where multiple users share one quantum computer, protecting user confidentiality becomes crucial. The varied uses of quantum computers increase the risk that sensitive data encoded by one user could be compromised by others, rendering the protection of data integrity and confidentiality essential. In the evolving quantum computing landscape, it is imperative to study these security challenges within the scope of realistic threat model assumptions, wherein an adversarial user can mount practical attacks without relying on any heightened privileges afforded by physical access to a quantum computer or rogue cloud services. In this paper, we demonstrate the potential of crosstalk as an attack vector for the first time on a Noisy Intermediate Scale Quantum (NISQ) machine, that an adversarial user can exploit within a multi-tenant quantum computing model. The proposed side-channel attack is conducted with minimal and realistic adversarial privileges, with the overarching aim of uncovering the quantum algorithm being executed by a victim. Crosstalk signatures are used to estimate the presence of CNOT gates in the victim circuit, and subsequently, this information is encoded and classified by a graph-based learning model to identify the victim quantum algorithm. When evaluated on up to 336 benchmark circuits, our attack framework is found to be able to unveil the victim's quantum algorithm with up to 85.7\% accuracy.

==> Tables/Bug_Details.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Details for the detected bugs in the benchmark SoC.}
\label{tab:bug-details}
\resizebox{\linewidth}{!}{%
\renewcommand{\arraystretch}{1}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{tabular}{@{}m{0.5cm}m{5.5cm}M{1.5cm}M{1.5cm}M{1.5cm}M{1.5cm}M{2.4cm}@{}}
\toprule
\multirow{2}{0.5cm}[-0.6em]{\centering\textbf{Bug No.}} 
& \multirow{2}{5cm}[-0.6em]{\centering\textbf{Bug Description}}
& \multirow{2}{1.5cm}[-0.6em]{\centering\textbf{Bug Location}}
& \multicolumn{2}{c}{\textbf{Sub modules involved}}
& \multirow{2}{1.5cm}[-0.6em]{\centering\textbf{CWE type}} 
& \multirow{2}{2.4cm}[-0.3em]{\centering\textbf{\# of input vectors needed to detect the bug}} \\ \cmidrule{4-5}

&
&
& \textbf{Sub-Module Name}
& \textbf{Total LOC}
&
& \\
\toprule
01. 
&  No feedback for data error in the Mailbox.
&  Mail-box
& \textit{scmi\_reg\_top}
&  735
&  *\textit{New Entry}*
& $6.47\times10^{6}$
\\ \midrule
02.  
& Key leakage into the bus using wipe command. 
& HMAC    
& \textit{hmac\_reg\_top}
& 1377     
& CWE-1258
& $7.82\times10^{6}$
\\ \midrule
03. 
&  No default state defined leading FSM to go into undefined state.
&  Life-Cycle Controller
& \textit{lc\_ctrl\_fsm}
&  735
&  CWE-1199
& $1.64\times10^{7}$
\\ \midrule
04.
& Enables production function before testing in unlocked states are completed.
& Life-Cycle Controller
& \textit{lc\_ctrl\_signal \_decoder}
& 384
& 
& $6.84\times10^{6}$
\\ \midrule
05.
& Key shares are leaked into the bus using key share offset commands.
& AES
& \textit{aes\_reg\_top}
& 1880
&  CWE-1342
& $6.97\times10^{6}$
\\ \midrule
06. 
& Bypassing one of the guard conditions of AES masking operations.
& AES
& \textit{aes}
& 300
&  CWE-1300
& $9.12\times10^{6}$
\\ \midrule
07. 
& Not clearing data registers with pseudo-random data.
& AES
& \textit{aes\_core} and \textit{aes\_cypher\_core}
& 1867
&  CWE-459
& $8.24\times10^{5}$
\\ \midrule
08. 
& AES masking operation with pseudo-random number is always off.
& AES
& aes\_prng \_masking
& 234
& CWE-1300
& $7.43\times10^{5}$
\\ \midrule
09. 
& Blanking operation in OTBN is disabled.
& OTBN
& otbn\_mac \_bignum
& 240
&  
& $8.32\times10^{6}$
\\ \midrule
10.
& ROM control skips checking state and goes into final state.
& ROM control
& \textit{rom\_ctrl\_fsm}
& 312
& 
& $6.82\times10^{6}$
\\ \midrule
11. 
& Power manager does not wait for the clear process to be finished.
& Power Manager
& \textit{pwr\_mgr\_fsm}
& 542
& CWE-1304
& $4.82\times10^{6}$
\\ \midrule
12. 
& Power manager does check ROM integrity check flag.
& Power Manager
& \textit{pwr\_mgr\_fsm}
& 542
& CWE-1304
& $4.82\times10^{6}$
\\ \midrule
13.
& The system cannot turn off parity check.
& UART
& \textit{uart\_rx}
& 137
&  
& $6.82\times10^{6}$
\\ \midrule
14. 
& Reseed Interval cannot be checked via the checker logic.
& CSRNG
& \textit{csrng\_reg\_top}
& 2042
&  
& $1.82\times10^{7}$
\\ \midrule
15. 
& Floating shadow register logic.
& Shadow Register
& prim\_subreg \_shadow
& 300
&  
& 
\\ \midrule
16. 
& System Reset Controller has the wrong value for the error flag.
& System Reset Control
& sysrst\_ctrl \_reg\_top
& 7218
&  
& 
\\ \midrule
17. 
& OTP controller clears data upon receipt of the \textit{enable} signal.
& OTP Controller
& otp\_ctrl\_dai
& 860
&  
& 
\\ \bottomrule
\end{tabular}%
}
\end{table*}

==> Tables/Comparison.tex <==
\begin{table}[t]
\centering
\caption{Bug Detected by the Fuzzers.}
\label{tab:bug-detect}
\resizebox{\linewidth}{!}{%
\renewcommand{\arraystretch}{1}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{tabular}{@{}M{1cm}M{1.2cm}M{1cm}M{1.2cm}M{1cm}@{}}
\toprule
\textbf{Bug No.}
& \textbf{\fram}
& \textbf{RFuzz}
& \textbf{DifuzzRTL}
& \textbf{HWFP} \\ \toprule
01.
& \cmark
& \xmark
& \xmark
& \xmark\\ \midrule
02.
& \cmark
& \cmark
& \cmark
& \cmark\\ \midrule
03.
& \cmark
& \xmark
& \cmark
& \cmark \\ \midrule
04.
& \cmark
& \xmark
& \cmark
& \cmark \\ \midrule
05.
& \cmark
& \xmark
& \xmark
& \xmark \\ \midrule
06.
& \cmark
& \cmark
& \cmark
& \cmark \\ \midrule
07.
& \cmark
& \xmark
& \xmark
& \xmark \\ \midrule
08.
& \cmark
& \xmark
& \xmark
& \xmark \\ \midrule
09.
& \cmark
& \xmark
& \cmark
& \cmark \\ \midrule
10.
& \cmark
& \xmark
& \cmark
& \cmark\\ \midrule
11.
& \cmark
& \xmark
& \xmark
& \xmark \\ \midrule
12.
& \cmark
& \xmark
& \cmark
& \cmark \\ \midrule
13.
& \cmark
& \xmark
& \cmark
& \xmark \\ \midrule
14.
& \cmark
& \cmark
& \xmark
& \xmark \\ \midrule
15.
& \cmark
& \cmark
& \cmark
& \cmark \\ \midrule
16.
& \cmark
& \xmark
& \cmark
& \xmark \\ \midrule
17.
& \cmark
& \xmark
& \cmark
& \cmark \\ \bottomrule
\end{tabular}%
}
\end{table}

==> Tables/Resource_Consumption.tex <==
\begin{table}[b]
\centering
\caption{Average Resource Consumption by Different Methods.}
\label{tab:avg_resource}
\resizebox{\linewidth}{!}{%
\renewcommand{\arraystretch}{1}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{tabular}{@{}m{2cm}M{3cm}M{2cm}@{}}
\toprule
\multicolumn{1}{c}{\textbf{Fuzzing Method}}
& \textbf{Memory Consumption (MB)}
& \textbf{CPU Usage (\%)} \\ \toprule
\fram
& 143
& 0.1 \\ \midrule
RFuzz
& 134
& 0.1 \\ \midrule
DifuzzRTL
& 137
& 0.15 \\ \midrule
HWFP
& 154
& 0.22 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> Tables/huzz_comparison.tex <==
\begin{table}[b]
\centering
\caption{Bug Detected by the Fuzzers.}
\label{tab:bug-huzz}
\resizebox{\linewidth}{!}{%
\renewcommand{\arraystretch}{1}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\begin{tabular}{@{}M{1cm}M{1.2cm}M{1cm}M{1.2cm}M{1cm}@{}}
\toprule
\textbf{Bug No.}
& \textbf{\fram}
& \textbf{HypFuzz}
& \textbf{PSOFuzz}
& \textbf{TheHuzz} \\ \toprule
V1
& \cmark
& \cmark
& \xmark
& \xmark\\ \midrule
V2
& \cmark
& \cmark
& \xmark
& \xmark \\ \midrule
V3
& \cmark
& \cmark
& \xmark
& \xmark \\ \midrule
V4
& \cmark
& \cmark
& \cmark
& \cmark \\ \midrule
V5
& \cmark
& \cmark
& \cmark
& \cmark \\ \midrule
V6
& \cmark
& \cmark
& \cmark
& \cmark \\ \midrule
V7
& \cmark
& \cmark
& \cmark
& \cmark \\ \midrule
V8
& \cmark
& \cmark
& \cmark
& \cmark \\ \midrule
V9
& \cmark
& \cmark
& \cmark
& \cmark \\ \midrule
V10
& \cmark
& \cmark
& \cmark
& \cmark \\ \bottomrule
\end{tabular}%
}
\end{table}
